A stochastic use of the Kurdyka-Lojasiewicz property: Investigation of optimization algorithms behaviours in a non-convex differentiable framework

Stochastic differentiable approximation schemes are widely used for solving high dimensional problems. Most of existing methods satisfy some desirable properties, including conditional descent inequalities, and almost sure (a.s.) convergence guarantees on the objective function, or on the involved gradient. However, for non-convex objective functions, a.s. convergence of the iterates, i.e., the stochastic process, to a critical point is usually not guaranteed, and remains an important challenge. In this article, we develop a framework to bridge the gap between descent-type inequalities and a.s. convergence of the associated stochastic process. Leveraging a novel Kurdyka-Lojasiewicz property, we show convergence guarantees of stochastic processes under mild assumptions on the objective function. We also provide examples of stochastic algorithms benefiting from the proposed framework and derive a.s. convergence guarantees on the iterates.

==> alphabet.tex <==
% Document LaTeX        GLB (25/05/94)
% Modification :        Gio (15/09/95)
%                       JI  (format Latex 2e, taille adaptative 22/03/99)
%                           (fonte blackboard 27/08/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{(necessite les packages xspace, amsmath, bbm)}
\typeout{}

\RequirePackage{amsmath}
\RequirePackage{xspace}
\RequirePackage{bbm}
%\RequirePackage{amssymb}
%\RequirePackage{bbold}
%\RequirePackage{mathbbol}
%\RequirePackage{doublestroke}

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
%\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)
\def\sbl#1{\ensuremath{\mathbb{#1}}}
\def\sbf#1{\ensuremath{\mathsf{#1}}}

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}

% Complément intéressant...

\def\ellb{\sbmm{\ell}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET \mathsf en math

\def\As{{\sbf{A}}\XS}  \def\as{{\sbf{a}}\XS}
\def\Bs{{\sbf{B}}\XS}  \def\bs{{\sbf{b}}\XS}
\def\Cs{{\sbf{C}}\XS}  \def\cs{{\sbf{c}}\XS}
\def\Ds{{\sbf{D}}\XS}  \def\ds{{\sbf{d}}\XS}
\def\Es{{\sbf{E}}\XS}  \def\es{{\sbf{e}}\XS}
\def\Fs{{\sbf{F}}\XS}  \def\fs{{\sbf{f}}\XS}
\def\Gs{{\sbf{G}}\XS}  \def\gs{{\sbf{g}}\XS}
\def\Hs{{\sbf{H}}\XS}  \def\hs{{\sbf{h}}\XS}
\def\Is{{\sbf{I}}\XS}  \def\is{{\sbf{i}}\XS}
\def\Js{{\sbf{J}}\XS}  \def\js{{\sbf{j}}\XS}
\def\Ks{{\sbf{K}}\XS}  \def\ks{{\sbf{k}}\XS}
\def\Ls{{\sbf{L}}\XS}  \def\ls{{\sbf{l}}\XS}
\def\Ms{{\sbf{M}}\XS}  \def\ms{{\sbf{m}}\XS}
\def\Ns{{\sbf{N}}\XS}  \def\ns{{\sbf{n}}\XS}
\def\Os{{\sbf{O}}\XS}  \def\os{{\sbf{o}}\XS}
\def\Ps{{\sbf{P}}\XS}  \def\ps{{\sbf{p}}\XS}
\def\Qs{{\sbf{Q}}\XS}  \def\qs{{\sbf{q}}\XS}
\def\Rs{{\sbf{R}}\XS}  \def\rs{{\sbf{r}}\XS}
\def\Ss{{\sbf{S}}\XS}  \def\ss{{\sbf{s}}\XS}
\def\Ts{{\sbf{T}}\XS}  \def\ts{{\sbf{t}}\XS}
\def\Us{{\sbf{U}}\XS}  \def\us{{\sbf{u}}\XS}
\def\Vs{{\sbf{V}}\XS}  \def\vs{{\sbf{v}}\XS}
\def\Ws{{\sbf{W}}\XS}  \def\ws{{\sbf{w}}\XS}
\def\Xs{{\sbf{X}}\XS}  \def\xs{{\sbf{x}}\XS}
\def\Ys{{\sbf{Y}}\XS}  \def\ys{{\sbf{y}}\XS}
\def\Zs{{\sbf{Z}}\XS}  \def\zs{{\sbf{z}}\XS}


% ALPHABET bold \mathsf en math

\def\Abs{{\boldsymbol{\sbf{A}}}\XS}  \def\abs{{\boldsymbol{\sbf{a}}}\XS}
\def\Bbs{{\boldsymbol{\sbf{B}}}\XS}  \def\bbs{{\boldsymbol{\sbf{b}}}\XS}
\def\Cbs{{\boldsymbol{\sbf{C}}}\XS}  \def\cbs{{\boldsymbol{\sbf{c}}}\XS}
\def\Dbs{{\boldsymbol{\sbf{D}}}\XS}  \def\dbs{{\boldsymbol{\sbf{d}}}\XS}
\def\Ebs{{\boldsymbol{\sbf{E}}}\XS}  \def\ebs{{\boldsymbol{\sbf{e}}}\XS}
\def\Fbs{{\boldsymbol{\sbf{F}}}\XS}  \def\fbs{{\boldsymbol{\sbf{f}}}\XS}
\def\Gbs{{\boldsymbol{\sbf{G}}}\XS}  \def\gbs{{\boldsymbol{\sbf{g}}}\XS}
\def\Hbs{{\boldsymbol{\sbf{H}}}\XS}  \def\hbs{{\boldsymbol{\sbf{h}}}\XS}
\def\Ibs{{\boldsymbol{\sbf{I}}}\XS}  \def\ibs{{\boldsymbol{\sbf{i}}}\XS}
\def\Jbs{{\boldsymbol{\sbf{J}}}\XS}  \def\jbs{{\boldsymbol{\sbf{j}}}\XS}
\def\Kbs{{\boldsymbol{\sbf{K}}}\XS}  \def\kbs{{\boldsymbol{\sbf{k}}}\XS}
\def\Lbs{{\boldsymbol{\sbf{L}}}\XS}  \def\lbs{{\boldsymbol{\sbf{l}}}\XS}
\def\Mbs{{\boldsymbol{\sbf{M}}}\XS}  \def\mbs{{\boldsymbol{\sbf{m}}}\XS}
\def\Nbs{{\boldsymbol{\sbf{N}}}\XS}  \def\nbs{{\boldsymbol{\sbf{n}}}\XS}
\def\Obs{{\boldsymbol{\sbf{O}}}\XS}  \def\obs{{\boldsymbol{\sbf{o}}}\XS}
\def\Pbs{{\boldsymbol{\sbf{P}}}\XS}  \def\pbs{{\boldsymbol{\sbf{p}}}\XS}
\def\Qbs{{\boldsymbol{\sbf{Q}}}\XS}  \def\qbs{{\boldsymbol{\sbf{q}}}\XS}
\def\Rbs{{\boldsymbol{\sbf{R}}}\XS}  \def\rbs{{\boldsymbol{\sbf{r}}}\XS}
\def\Sbs{{\boldsymbol{\sbf{S}}}\XS}  \def\sbs{{\boldsymbol{\sbf{s}}}\XS}
\def\Tbs{{\boldsymbol{\sbf{T}}}\XS}  \def\tbs{{\boldsymbol{\sbf{t}}}\XS}
\def\Ubs{{\boldsymbol{\sbf{U}}}\XS}  \def\ubs{{\boldsymbol{\sbf{u}}}\XS}
\def\Vbs{{\boldsymbol{\sbf{V}}}\XS}  \def\vbs{{\boldsymbol{\sbf{v}}}\XS}
\def\Wbs{{\boldsymbol{\sbf{W}}}\XS}  \def\wbs{{\boldsymbol{\sbf{w}}}\XS}
\def\Xbs{{\boldsymbol{\sbf{X}}}\XS}  \def\xbs{{\boldsymbol{\sbf{x}}}\XS}
\def\Ybs{{\boldsymbol{\sbf{Y}}}\XS}  \def\ybs{{\boldsymbol{\sbf{y}}}\XS}
\def\Zbs{{\boldsymbol{\sbf{Z}}}\XS}  \def\zbs{{\boldsymbol{\sbf{z}}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}


% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\varkappab   {{\sbmm{\varkappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}     \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}         \def\Xib       {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}         \def\Pib       {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}   \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib      {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib      {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}    \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}

% ALPHABET GREC GRAS droit, taille adaptative

\def\alphav      {{\sdm{\alpha}}\XS}
\def\betav       {{\sdm{\beta}}\XS}
\def\gammav      {{\sdm{\gamma}}\XS}      \def\Gammav    {{\sdm{\Gamma}}\XS}
\def\deltav      {{\sdm{\delta}}\XS}      \def\Deltav    {{\sdm{\Delta}}\XS}
\def\epsilonv    {{\sdm{\epsilon}}\XS}
\def\varepsilonv {{\sdm{\varepsilon}}\XS}
\def\etav       {{\sdm{\eta}}\XS}
\def\thetav      {{\sdm{\theta}}\XS}      \def\Thetav    {{\sdm{\Theta}}\XS}
\def\varthetav   {{\sdm{\vartheta}}\XS}
\def\iotav       {{\sdm{\iota}}\XS}
\def\kappav      {{\sdm{\kappa}}\XS}
\def\varkappav   {{\sdm{\varkappa}}\XS}
\def\lambdav     {{\sdm{\lambda}}\XS}     \def\Lambdav   {{\sdm{\Lambda}}\XS}
\def\muv         {{\sdm{\mu}}\XS}
\def\nuv         {{\sdm{\nu}}\XS}
\def\xiv         {{\sdm{\xi}}\XS}         \def\Xiv       {{\sdm{\Xi}}\XS}
\def\piv         {{\sdm{\pi}}\XS}         \def\Piv       {{\sdm{\Pi}}\XS}
\def\varpiv      {{\sdm{\varpi}}\XS}
\def\rhov        {{\sdm{\rho}}\XS}
\def\varrhov     {{\sdm{\varrho}}\XS}
\def\sigmav      {{\sdm{\sigma}}\XS}      \def\Sigmav    {{\sdm{\Sigma}}\XS}
\def\varsigmav   {{\sdm{\varsigma}}\XS}   \def\Varsigmav {{\sdm{\Varsigma}}\XS}
\def\phiv      {{\sdm{\phi}}\XS}        \def\Phiv     {{\sdm{\Phi}}\XS}
\def\varphiv     {{\sdm{\varphi}}\XS}
\def\chiv        {{\sdm{\chi}}\XS}
\def\psiv        {{\sdm{\psi}}\XS}        \def\Psiv      {{\sdm{\Psi}}\XS}
\def\omegav      {{\sdm{\omega}}\XS}      \def\Omegav    {{\sdm{\Omega}}\XS}
\def\tauv        {{\sdm{\tau}}\XS}
\def\upsilonv    {{\sdm{\upsilon}}\XS}    \def\Upsilonv  {{\sdm{\Upsilon}}\XS}
\def\zetav       {{\sdm{\zeta}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}
\def\eI{\Ibb}
\def\eB{\Bbb}
\def\eV{\Vbb}
\def\eL{\Lbb}
